No-Frills Human-Object Interaction Detection: Factorization, Layout Encodings, and Training Techniques

We show that for human-object interaction detection a relatively simple factorized model with appearance and layout encodings constructed from pre-trained object detectors outperforms more sophisticated approaches. Our model includes factors for detection scores, human and object appearance, and coarse (box-pair configuration) and optionally fine-grained layout (human pose). We also develop training techniques that improve learning efficiency by: (1) eliminating a train-inference mismatch; (2) rejecting easy negatives during mini-batch training; and (3) using a ratio of negatives to positives that is two orders of magnitude larger than existing approaches. We conduct a thorough ablation study to understand the importance of different factors and training techniques using the challenging HICO-Det dataset.

==> Tables/factor_ablation_all_cols.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \addtolength{\tabcolsep}{0pt}
    \begin{tabular}{lccccccccc}
        \toprule
        & \multirow{2}{*}{\textbf{Full}}  & \multirow{2}{*}{\textbf{Rare}}  & \multirow{2}{*}{\textbf{Non-Rare}} & \multicolumn{6}{c}{\textbf{Number of training instances per HOI class}} \\
        \cmidrule(r){5-10}
        &&&                        & \textbf{0-9}   & \textbf{10-49} & \textbf{50-99} & \textbf{100-499} & \textbf{500-999} & \textbf{1000+} \\
        \midrule
        HO-RCNN~\cite{chao2017hicodet}   & 7.81  & 5.37  & 8.54     & -     & -     & -     & -       & -       & -     \\
        VSRL~\cite{gupta2015vsrl} (impl. by ~\cite{gkioxari2017hoi})       & 9.09  & 7.02  & 9.71     & -     & -     & -     & -       & -       & -     \\
        InteractNet~\cite{gkioxari2017hoi} & 9.94  & 7.16  & 10.77    & -     & -     & -     & -       & -       & -     \\
        GPNN~\cite{qi2018graphparsingnn} & 13.11  & 9.34  & 14.23    & -     & -     & -     & -       & -       & -     \\
        iCAN~\cite{Gao2018iCANIA} & 14.84  & 10.45  & 16.15    & -     & -     & -     & -       & -       & -     \\ 
        \midrule
        Det                    & 8.32  & 6.84  & 8.76  & 6.84  & 4.85  & 6.05  & 10.18 & 14.40 & 21.46 \\
        Det + Box              & 12.54 & 10.40 & 13.18 & 10.40 & 7.46  & 9.99  & 14.62 & 20.12 & 35.98 \\
        Det + Human App        & 11.12 & 8.82  & 11.80 & 8.82  & 7.73  & 9.19  & 13.41 & 15.85 & 26.42 \\
        Det + Object App       & 11.05 & 7.41  & 12.13 & 7.41  & 7.68  & 9.72  & 14.61 & 15.58 & 23.27 \\
        Det + App              & 15.74 & 11.35 & 17.05 & 11.35 & 10.58 & 13.96 & 20.11 & 22.76 & 34.75 \\
        Det + Human App + Box  & 15.63 & \red{12.45} & 16.58 & \red{12.45} & 9.94  & 12.69 & 19.05 & 23.60 & 39.63 \\
        Det + Object App + Box & 15.68 & 10.47 & 17.24 & 10.47 & 9.97  & 12.84 & 20.48 & 23.88 & 40.87 \\
        Det + App + Box        & \blue{16.96} & 11.95 & \blue{18.46} & 11.95 & \blue{11.02} & \blue{14.00} & \blue{22.02} & \blue{25.01} & \blue{41.13} \\
        \midrule
        Det + Pose             & 11.09 & 8.04  & 12.00 & 8.04  & 7.26  & 8.47  & 13.08 & 18.81 & 32.66 \\
        Det + Box + Pose       & 14.49 & 11.86 & 15.27 & 11.86 & 9.73  & 12.21 & 16.51 & 21.72 & 38.81 \\
        Det + App + Pose       & 15.50 & 10.14 & 17.10 & 10.14 & 10.40 & 13.11 & 20.40 & 23.45 & 36.08 \\
        Det + App + Box + Pose & \red{17.18} & \blue{12.17} & \red{18.68} & \blue{12.17} & \red{11.28} & \red{14.49} & \red{22.08} & \red{25.27} & \red{41.47} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Results on HICO-Det test set.} Det, Box, App, and Pose correspond to object detector terms, appearance, box configuration, and pose factors respectively. Each row was both trained and evaluated with specified factors. \red{Best} and \blue{second best} numbers are highlighted in color.}
    \label{tbl:ch4_factor_ablation}
\end{table*}
    
